Enhanced stability of pressure relief valves: mechanistic design and analysis

Pressure-relief valves, often the critical last line of defence in process engineering, are known to be susceptible to valve chatter. Such behaviour has been shown to arise from a flutter instability, or Hopf bifurcation, associated with the fundamental, quarter-wave acoustic mode of their inlet piping. Here, a novel design concept is proposed and analyzed for eliminating this instability. The concept involves using an oversized valve with reduced lift and adopting a discharge characteristic that enhances the blow-down effect, so that the valve opens immediately to its upper lift limit upon reaching set pressure. The concept is demonstrated numerically using an updated version of a 1D fluid pipe dynamics mathematical model solved using a Lax-Wendroff method. Stability properties are analysed using dynamical systems theory, applied to an improved reduced-order modal model. It is shown how the valve settles to a stable so-called pseudo equilibrium, in contact with the upper stop, provided the coefficient of restitution of is not too large. Such stable operation is reached despite the equivalent regular valve being unstable to the quarter-wave Hopf bifurcation. Parameter studies using the reduced-order model demonstrate the extent of the enhanced stability effect, which is confirmed using the full model for the case of gas service valves.

==> graphicalAbstract.tex <==
\begin{frontmatter}
\begin{graphicalabstract}
	%	\begin{figure}
		\begin{minipage}{0.35\textwidth}
			\begin{center}
				\ \\[-1cm]
				\includegraphics[width = 0.95 \linewidth] {restricted_valve} \\[-1.5cm]
				{\scriptsize Schematic of novel valve design.}
			\end{center}
		\end{minipage}
		\begin{minipage}{0.6\textwidth}
			\begin{center}
				\ \\[0.5cm] 
				\includegraphics[width = 0.8\linewidth]{Aeff-virtual-demo-four-stages} \\
				{\scriptsize Lift-versus pressure characteristic in the presence of restricted lift, showing a typical superimposed pressure relief event. }
			\end{center}
		\end{minipage}  \\[0.5cm] 
		%
		\begin{center}        
			\includegraphics[width = 0.45\linewidth]{chi-Lambda-1WM-stability-front}	\hspace{1 cm}
			\includegraphics[width = 0.45\linewidth]{2J3_Aeff_NL_chi_1_Stability_bound_front}	\\
			{\scriptsize Left: Stability chart of original design. Right: novel design. Green circles show stability, red crosses instability. Solid line analytic approximation to stability boundary.   }
		\end{center}
		%{\color{red}ARC: need to create a new version of this figure where we remove the red and blue lines from this figure, the key, the triangles and the labels (a) and (b)}
		%
	\end{graphicalabstract}
	\end{frontmatter}

==> highlights.tex <==
\begin{frontmatter}
%%Research highlights
\begin{highlights}
	\item A new design concept greatly enhances stability of pressure-relief valves against flutter and chatter instability.
    \item The design exploits interaction between fold and Hopf bifurcations, and nonsmooth andalysis of contacting pseudo equilibria. 
	\item Practical implementation is proposed either using oversized valves with restricted lift, or via novel equilibrium-versus-lift characteristics. 
	\item An experimentally validated coupled pipeline-valve model is improved to deal with the new design.
	 \item Detailed steady and transient simulations verify wide parameter sets for which stable oscillation is achieved.
\end{highlights}
	\end{frontmatter}

==> title.tex <==
\begin{frontmatter}
	
\title{Enhanced stability of pressure relief valves: mechanistic design and analysis}

%% use optional labels to link authors explicitly to addresses:
%% \author[label1,label2]{}
%% \affiliation[label1]{organization={},
	%%             addressline={},
	%%             city={},
	%%             postcode={},
	%%             state={},
	%%             country={}}
%%
%% \affiliation[label2]{organization={},
	%%             addressline={},
	%%             city={},
	%%             postcode={},
	%%             state={},
	%%             country={}}

\author[inst1]{Hong Tang}

\affiliation[inst1]{organization={Department of Engineering Mathematics,University of Bristol},%Department and Organization
	addressline={Queen's Building},
	city={Bristol},
	postcode={BS1 8TH},
	%state={},
	country={UK}}

\author[inst2]{Istvan Erdodi}

\author[inst1]{Alan R. Champneys}

%\newunicodechar{ű}{\H{u}}
%\newunicodechar{ő}{\H{o}}

\author[inst2]{Csaba J. H{ő}s}

\affiliation[inst2]{organization=
	{Department of Hydrodynamic Systems, Budapest University of Technology and Economics},
	addressline={M{ű}egyetem rkp. 3.},
	city={Budapest},
	postcode={1111},
	%state={State Two},
	country={Hungary}
}

\input{Abstract.tex}
\begin{keyword}
	%% keywords here, in the form: keyword \sep keyword
	pressure-relief valve \sep stability enhancement \sep qurater-wave instability \sep blowdown \sep valve chatter \sep pipeline dynamics 
	%% PACS codes here, in the form: \PACS code \sep code
	\PACS 47.85.L- \sep 46.32.+x
	%% MSC codes here, in the form: \MSC code \sep code
	%% or \MSC[2008] code \sep code (2000 is the default)
	\MSC 35L35 \sep 37N10
\end{keyword}

\end{frontmatter}
